Backscattering-free edge states below all bands in two-dimensional auxetic media

Unidirectional and backscattering-free propagation of sound waves is of fundamental interest in physics, and highly sought-after in engineering. Current strategies utilize topologically protected chiral edge modes in bandgaps, or complex mechanisms involving active constituents or nonlinearity. Here we propose a new class of passive, linear, one-way edge states based on spin-momentum locking of Rayleigh waves in two-dimensional media in the limit of vanishing bulk modulus, which provides $100\%$ unidirectional and backscattering-free edge propagation at a broad range of frequencies instead of residing in gaps between bulk bands. We further show that such modes are characterized by a new topological winding number that is analogous to discrete angular momentum eigenvalues in quantum mechanics. These passive and backscattering-free edge waves have the potential to enable a new class of phononic devices in the form of lattices or continua that work in previously inaccessible frequency ranges.

==> commands.tex <==
\newcommand{\edge}{r}
\newcommand{\edgevector}{\mathbf{\edge}}
\newcommand{\edgedirection}{\hat{\edge}}

\newcommand{\springconstant}{k}

\newcommand{\displacement}{\mathbf{U}}
\newcommand{\force}{\mathbf{F}}

\newcommand{\tension}{t}
\newcommand{\tensionvector}{\mathbf{\tension}}
\newcommand{\equilibriummatrix}{\mathbf{A}}
